A Conditional Generative Matching Model for Multi-lingual Reply Suggestion

We study the problem of multilingual automated reply suggestions (RS) model serving many languages simultaneously. Multilingual models are often challenged by model capacity and severe data distribution skew across languages. While prior works largely focus on monolingual models, we propose Conditional Generative Matching models (CGM), optimized within a Variational Autoencoder framework to address challenges arising from multi-lingual RS. CGM does so with expressive message conditional priors, mixture densities to enhance multi-lingual data representation, latent alignment for language discrimination, and effective variational optimization techniques for training multi-lingual RS. The enhancements result in performance that exceed competitive baselines in relevance (ROUGE score) by more than 10\% on average, and 16\% for low resource languages. CGM also shows remarkable improvements in diversity (80\%) illustrating its expressiveness in representation of multi-lingual data.

==> Sections/ethical_discussion.tex <==
\section*{Ethical Considerations}
The primary ethical concern in our paper is the use of Reddit data for training, evaluation, and creation of response sets, from which we derive our insights and conclusions about the proposed algorithms. While the source Reddit dataset from pushift.io \cite{baumgartner2020pushshift} has been used in numerous peer reviewed publications, there are many issues that we need to acknowledge and be aware of. Prior work has revealed that content and conversation in Reddit can be inappropriate, and abusive \citep{massanari2017gamergate,mohan2017impact}. In addition the conversations can have racial or gender biases, and may contain contributions from bots, paid users, and many forms of spams. All these issues can conflate or bias the results shown in this paper. 

While we have done due diligence to clean the content, we do not recommend the use of approaches in this paper (and the released code) with the Reddit datasets from Pushift for any scenario involving real users or products. We also believe that usage of the data for human annotations is not appropriate without careful curation of evaluation messages, the response sets, and the predicted responses, as it can expose the inappropriate content and biases to human users. 

We present some text samples of predictions (with messages created by authors), using the response sets generated from the Reddit set. However, we removed any sample response which we considered as blatantly inappropriate before presenting in this paper. Fortunately there were very few such instances in the samples but it does alert us to the fact that the data cannot be used for large scale human evaluations as is. We have also presented samples in languages other than English, for which are not the native language of any of the authors. We used machine translation to evaluate these samples, but acknowledge that we are unable to completely judge the appropriateness of these samples. 

Finally, while we have used the terminology of "universal multilingual models" as a motivation for spreading the technology across the regions of the globe, only 15 languages used here cover a very small portion of mostly European languages, let alone the world. We acknowledge this lack of equitable coverage of more languages, and the use of phrase "universal multilingual models" should be used with a caveat.
